Commonsense Knowledge in Word Associations and ConceptNet

Humans use countless basic, shared facts about the world to efficiently navigate in their environment. This commonsense knowledge is rarely communicated explicitly, however, understanding how commonsense knowledge is represented in different paradigms is important for both deeper understanding of human cognition and for augmenting automatic reasoning systems. This paper presents an in-depth comparison of two large-scale resources of general knowledge: ConcpetNet, an engineered relational database, and SWOW a knowledge graph derived from crowd-sourced word associations. We examine the structure, overlap and differences between the two graphs, as well as the extent to which they encode situational commonsense knowledge. We finally show empirically that both resources improve downstream task performance on commonsense reasoning benchmarks over text-only baselines, suggesting that large-scale word association data, which have been obtained for several languages through crowd-sourcing, can be a valuable complement to curated knowledge graphs

==> body/__latexindent_temp.tex <==
 
\section{Introduction}

% What is the problem?
% ConceptNet is a giant and sparse, it doesn't translate to other language easily
% SWOW is small but dense with a simpler architecture, SWOW is easier to transfer to other language

%p1: commonsense knowledge graph is important, 对谁重要，为何重要， 
% why commonsense knowledge is important? It's important for what ? 
% Collecting commonsense knowledge is challenging?


Commonsense reasoning is 
and association 
The ability to  
Given an commonsense question  
people can easily associate key concepts in a question with the correct answer 
For example, if we observe (Fig 1), we can easily 

Teaching machines to 
Commonsense knowledge is vital for natural language understanding. 
Many tasks have shown that 
question answering, 
dialogue systems, 
story understanding, 
require commonsense reasoning about the world 
To answer a question like "" require a model to draw on world knowledge like "". 
%select a example

% Without commonsense knowledge, it is challenging for a model to answer questions requiring knowledge beyond given texts. 
% Missing commonsense knowledge making it challenging for a model to answer questions requiring knowledge beyond given texts. 
% require the model to use commonsense knoweldge rather than just co-occurance information to answer the question. 

%main claim: commonsense knowledge is important for commonsense question  answering

%p2: commonsense knowledge collection method
Commonsense knowledge in ConceptNet are usually collected in three ways, including hand-crafted by experts, automatically extracted from the Web, and games with a purpose. 

%p2: ConceptNet is sparse, making it difficult to learn knowledge graph embeddings 
% ConceptNet is huge, and heavy, big? 
Existing models use commonsense knowledge graph as additional source to assist downstream tasks. 
Nodes and relations in a knowledge graph are represented as embeddings and are incorporated to question-answer models.
However, train high quality knowledge graph embeddings models often require the graph is densely connected to learn better representations.
ConceptNet is a giant semantic network containing commonsense facts. 
It has been shown that it is  useful for improving accuracy of many NLP tasks.
However, it is sparse and  
Knowledge in ConceptNet is collected from three ways: hand-crafted by experts, automatically extracted from the Web, and games with a purpose. which is either time and money consuming or hard to capture the unstated commonsense. 

Creating a massive commonsense knowledge graph like ConceptNet in other languages are unrealistic. 


%p3: Word Associations contain commonsense knowledge, it has not been used before
% why word association can be seen as or used as commonsense knowledge?
% 1). Even though no specific relation are specified, word associations is similar to games with a purpose, which is privously used for collecting commonsense knoweldge and is one of the source in ConceptNet. 
% 2). Word associations is also related to property norms that aksing humans 
% 2). Word associations is collected from volunteers, and thus it contain the knowledge elicited from human,  
 
% games can be used to collect common sense facts, 
% uses templates to question players about goals
% commonsense facts -> gather commonsense facts through Games with a purpose ->
% 
% common sense facts, games with purpose
% ConceptNet has a similar setup as 
% commonsense associations 

Another manner of 
One knowledge source of ConceptNet is word associations from purposes with a game, like Verbosity, 
collecting commonsense associations from a large auidence of ordinary humans by playing games. 
Relations associate two words are categoried by different sentence templates, 
%such as `\___ is used for \___.'. 
And property norms
Another form of association is free word associations, revealing how human build mental representations for concepts around us in our daily life.  
 humans to respond with any word associated with the given cue word. 
It makes the collection process become less effortlessly for paricipants and elicits more deeply and broadly associations in human minds without the speficied relation restriction.
%we focus on SWOW
By crowd-sourcing, large-scale free word association resource SWOW \citep{Deyne2013BetterEO,Deyne2019TheW} is curated.
This resource contains valuable knowledge, surprsingly, its utility for natural language understading has not been explored.

% What are your contributions?
In this paper, we explore the utility of commonsense knowledge collected from free associations for commonsense question answering, by representing it as knowledge graph embeddings and applying it to downstream tasks. 
Also, we compare it to ConceptNet to study which one is more useful for commonsense question answering.
Our main contributions are:
\begin{itemize}
    \item We show that the free word association network SWOW alone can be used for answering commonsense questions.
    \item We show that incorporating SWOW improves on baseline question-answering models on a couple of commonsense question answering tasks.  
    \item We compare the utility of ConceptNet and SWOW from both qualitative and quantitative aspects, showing that SWOW brings more improvements to xx tasks, while ConceptNet contribute more to yy tasks. 
    % 我们从x,x,x,方面对比了  SWOW 和 ConceptNet 对downstream tasks 的影响，发现在y1方面swow bring more benefits than concept.
\end{itemize}


\section{Commonsense Knowledge}
\begin{table*}[t]
    \centering
    \begin{tabular}[width=\textwidth]{lccccccc}
    	\toprule
    	\textbf{KG} & \textbf{Triples} & \textbf{E} & \textbf{R} & \textbf{D} & \textbf{ID} & \textbf{EE} & \textbf{RE} \\
    	\midrule
    	ConceptNet & 2,403,453 & 799,273 & 17 & 3.76e-06 & 2.95 & 4.73 & 1.0e-4\\
        SWOW & 1,595,556 & 124,627 & 2 & 1.03e-04 & 11.11 & 1.11 & 1.79e-05\\
        % \hline 
        % SWOW497K & 497,516 & 34,398 & 2 & 4.20e-04 & 11.99 & 0.91 & 5.27e-05\\
    	\bottomrule
    \end{tabular}
    \caption{\label{tab:statitics_cn_rel17_sw} Statistics of ConceptNet5.6 and SWOW. To densify the graph for better knowledge graph training, 47 relation types are merged into 17 types \citep{Lin2019KagNetKG}. E and R are unique entity and relation numbers. D is the graph density. ID is the average in-degree nodes. EE and RE are the entity entropy and relation entropy.}
\end{table*}  

% Focus on the comparisons of them, both statistical numbers and also the contents (why we want to use SWOW)
% I want to show my readers that SWOW is an promising resources for commonsense reasoning. 
% I need to show 
% what is SWOW (how does it come from) 
% the differences between them, 
% the advantages of SWOW.  
% why SWOW is suitable for commonsense reasoning 

\subsection{ConceptNet Knowledge Collection}
ConceptNet \citep{Speer2017ConceptNet5A}, originated from Open Mind Common Sense (OMCS) (Singh, 2002) project launched in 1999, is presently the largest knoweldge graph containing relational commonsense knowledge.  
To expand the knowledge beyond OMCS, the recent version, ConceptNet5.5 (Speer et al., 2017) integrates knowledge from several additional sources, such as Wiktionary. 
Each node in the graph is an arbitrary natural language phrase or word, and each edge is labelled with a semantic relation, e.g., `UsedFor, PartOf'.
These semantic relational facts are useful for answering commonsene questions as can help determine the plausiabilty of a given answer choice.
% The free-text form of nodes increasing its number tremendously, but the connections among them are not sufficient, making it suffers high sparsity.
% It has since grown to include knowledge from other crowdsourced resources, expert-created resources, and games with a purpose.
% collecting and integrating data from many years since the beginning of the MIT Open Mind Common Sense project
% Cyc (Lenat et al., 1985), WordNet (Fellbaum, 1998) and DBpedia (Auer et al., 2007). 
% For this reason, ConceptNet has a wider spectrum of semantic relationships but a much more sparse coverage.
%%%%


\subsection{SWOW Knowledge Collection}
%How SWOW is created, how do I make use of it?
SWOW \citep{Deyne2019TheW} is currently the largest word association collection in English, collected between 2011 to 2018 from over 9,000 participants.
It captures general associations among English nouns, adjectives, verbs and adverbs.

After pre-processing, we obtain xxx unique cues and xxx responses with xxx edges.
The current released SWOW-EN consists repsonses from 100 participants per cue, and each participant can generate at most 3 responses. This process resulting in a graph that is densely connected.
% with 12,217 cues and 3,665,100 responses 
As SWOW is not labelled with relation types, to train it with knowledge graph embedding techniques like TransE, we label edges with directionality of association, including \textit{forward association, backward association, and mutual association}. 

%Why it can be used for commonsense reasoning: its large scale and high density 

\subsection{A surface Comparison}
The difference between \texttt{ConceptNet} and \texttt{SWOW} is that the former contains semantic relations, such as `PartOf, UsedFor, IsA', while the latter contains more general associations among words under the broad category of `use', `form' and `meaning' \citep{Nation2001LearningVI}. 
They share common nodes and also have their own biases. 
% knowledge quality is very good, and the rate of knowledge collection is rapid

ConceptNet 
    花了很多年构建, 
    稀疏，automatic construction,
    包含relations (适合commonsense reasoning的),  


SWOW: 目前是7年,
    比ConceptNet密 (尤其是cue words的connection 以及single word的connections[collocations比ConceptNet多]),没有relations, crowdsourcing
    increase scability

In contrast to ConceptNet, 

SWOW could complement ConceptNet in terms of 
In light of this, exploring whether word associations network can be used as an usable  


%%%
SWOW and ConceptNet have several similarities: 
(1) they both contain general commonsense knowledge (); 
and 
(2) concepts in the two graphs are both in the form of natural language and their ambiguities are not diffierentiated;

On the other hand, SWOW and ConceptNet differ from each other in some aspects: 
(1) ConceptNet is a relational semantic network, however, SWOW doesn't contain relational edges and the latent realtion types of word association could be different from semantic relations in ConceptNet;
(2) as their processes of development differ (manually handcrafted vs. automatically generated), intuitively ConceptNet has higher quality and robustness;
(2) while ConceptNet contains more compound concepts 
while WordNet focuses on formal taxonomies of words, ConceptNet focuses on a richer set of semantic relations between compound concepts [6]; 
and (3) WordNet differentiates ambiguous meanings of a word as synsets, however, ConceptNet bears
ambiguity of commonsense knowledge in its concepts and relations. 
% Most work that uses ConceptNet as external knoweldge graph rely on relation information for modeling, however, which is obsent from SWOW, making its incorporation become unfeasible. 

\section{Models}

To study the utility of of a knowledge graph to downstream commonsense reasoning tasks, we pre-train it with knowledge graph embedding techniques and use it to augment vanilla question answering models.

To examine the effectiveness of a knowledge graph under different settings, three groups of encoders are used for representing a pair of question and answer, including graph model and text+graph model. 

\textbf{KG models}
To investigate whether knowledge from a knowledge graph alone can be used to answer questions, we use KG-aware models to encode question-answer relevant knowledge retrieved from a knowledge graph for question answering.
Naturally, a KG-aware model generates a knowledge embedding $\mathrm{k}$ to represent structure information for classification.
To compare ConceptNet and SWOW throughly, we employ different types of KG-aware models, ranging from static KG-aware models, i.e., GconAttn and RN, to dynamic KG-aware models i.e., PG-Global and PG-Full. 


\textbf{GconAttn} \citep{Wang2019ImprovingNL} aligns grounded question concepts and answer concepts with concept-level attention and pooling strategy to generate a fixed knowledge embedding $\mathrm{k}$. 
This model only incorporates graph structure and entity representation for modeling and without assuming the access to relations, thus it is a relation free model. 

\textbf{RN} \citep{Santoro2017ASN} generates knowledge embedding$ \mathrm{k}$ by performing path-level attention over paths retrieved from a KG for each pair of question-answer entities. 
% RN attention over retrieved paths for each pair of question-answer entities from a static KG to obtain a static KG embedding
As paths serve as structure message, RN is an relation dependent model. 

\textbf{PG-Global} \citep{Wang2020ConnectingTD} generates dynamic knowledge embedding $k$ with a pre-trained path generator, which is a fine-tuned GPT-2 with  multi-hop paths sampled from a KG. %, i.e., ConceptNet or SWOW.

\textbf{PG-Full} \citep{Wang2020ConnectingTD}, a strong model for commonsense question answering, unifies static knowledge embedding from RN and dynamic knowledge embedding from PG-Global. 


% The concept embeddings are trained with knowledge graph embedding techniques. We choose the representative of distance-based model TransE and the semantic similarity-based model DistMult for training.


\textbf{Text Models} 
% Text encoder encodes textual information in the given question and answer.
We explore a range of text encoder, including a simple encoder BiGRU and pre-trained language models BERT-Base and Albert. 
BiLSTMs learns the contextual representations for a pair of question and answer.
The text encoder takes input of a single sequence concatenated by a question and an answer and outputs a fixed dimension vector for answer scoring. 
In addition, previous researches have shown that fine-tuning pre-trained language models like BERT, achieve promising performances on commonsense question answering tasks.  
So, we also use BERT-Base and RoBERTa as sentence encoders to examine
whether knowledge from external knowledge graph like SWOW can bring information beyond pre-trained language model and textual information. 

\textbf{Text+KG Models}
To augment text representation with knowledge representation, we experiment with adding graph models on top of text models. Specifically, we concatenate  representations from the text encoder and graph encoder for final classification. 

\section{Experiments}
\subsection{Datasets}
\begin{table}
    \begin{adjustbox}{width=0.5\textwidth}
    \small
    \begin{tabular}[width=\textwidth]{lcccc}
        \toprule
         & Train & Dev & Test & C \\
        \midrule
        CommonsenseQA & 8,500 & 1,221 & 1,241 & 5 \\
        OpenBookQA & 4,957 & 500 & 500 & 4 \\
        % SocialIQA & 33,410 & 1,954 & 2,224 & 3 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\label{tab:datasets_statistics} Statistics of three commonsense question answering datasets.* uses the split from \citep{Lin2019KagNetKG}. C denotes the number of choices.}
\end{table}

We consider two commonsense question answering datasets for experiments. 
They all are  multiple-choice style, and crated to prob the commonsense reasoning ability of a model. Statistics of the two datasets are shown in Table~\ref{tab:datasets_statistics}. \\
% crowdsourced
%What properties does CommonsenseQA(descriptions) have and why it is challenging?
\textbf{CommonsenseQA} \citep{Talmor2019CommonsenseQAAQ} contains commonsense questions generated based on sub-graphs extracted from ConceptNet by crowd-workers.
Answering questions in this dataset is challenging as it requires various commonsense skills, and it's difficult to distinguish distractors from the correct answer because they often share same semantic relations as the key concepts in a question.
% $and also answering its questions require various commonsense skills.
% requiring a model to draw on the knowledge beyond text for help
% require general background knowledge to answer these questions 

\textbf{OpenBookQA} \citep{Mihaylov2018CanAS} contains questions along with elementary level science facts built from open book exams. It requires a model to combine book knowledge and commonsense knowledge for reasoning. In this work, we ignore the provided facts and use knowledge extracted from ConceptNet and SWOW as background knowledge.
% SocialIQA \citep{Sap2019SocialIC} collects commonsense reasoning questions in social situations. [add one more sentence]

\subsection{Experimental setup}

% \paragraph{Path Sampling}
% Paths are sampled from a KG with random walk 
% for training dynamic path generator, we use  
% To enrich the knowledge graph and allow entities 
% We add a reverse relation $r^{-1}$ for each relation $r$


\paragraph{KG Embeddings}
We employ pre-trained language model RoBERTa to extract entity embeddings. 
Specifically, for each entity $e_i$, we feed the sequence of $[‘CLS’, e_i, ‘SEP’]$ to RoBERTa and then use the representation of ‘CLS’ token from the last layer to represent its entity embedding. 
We use relation embeddings pre-trained on a knowledge graph with TransE \footnote{TransE is trained with OpenKE https://github.com/thunlp/OpenKE}.



% The dimension of entity and relation embeddings for TransE and DistMult is 100. The hidden dimension for lstm as text encoder is 128, and graph encoder is 64. 
% We use OpenEA\footnote{https://github.com/thunlp/OpenKE} to train knowledge graph embeddings. 


\begin{comment}


\subsection{Results on Commonsense Question Answering} 
In the next section we will answer the following questions: \\
% \begin{itemize}
\textbf{Q1}. Can knowledge graph embeddings trained on SWOW be used to perform commonsense question answering?\\ %KG > random, KG vs Text     
\textbf{Q2}. Can knowledge graph in SWOW bring additional improvements on text encoder?\\
\textbf{Q3}. How does knowledge retrieved from ConceptNet and SWOW is different?\\ %(The pros and cons of CN and SW) 
% \end{itemize}

% We can also see that TransE is perform xx than DistMult on xx datasets, which may because of 

% On average, premise and hypothesis sentences consist of 19 and 12 words respectively, but their respective One-Hop graphs have over
% Avg Concepts Premise (19 words) % 9 369 23
% Avg Concepts Hypothesis (12 wordso


\subsubsection{Ablation}
%what kinds of knowledge beyond text are in ConceptNet and SWOW? 
To better understand why SWOW can achieve similar improvements on three datasets.
We study the difference of ConceptNet and SWOW in terms of the coverage and representation of mentioned concepts over three datasets.

For the coverage, we did statistics for mentioned concept types and tokens over three datasets. We found that even though SWOW has lower type coverage than ConceptNet, the token coverage is almost identical, which could explain that why they obtain similar improvements.

Furthermore, to investigate how coverage influences the performance to downstream tasks. 
For both concepts in SWOW and ConceptNet,
We use the

One concern of using SWOW as a knowledge base is that its concepts coverage is much lower than ConceptNet, which may weaken its influence to downstream tasks.
So we compare the statistics of mentioned concepts from two knowledge graphs on three datasets, shown in Table~\ref{tab:retrieved_concepts_statistics}.
We can see that even less mentioned concepts are retrieved from SWOW, it still performs better than ConceptNet, suggesting that its densely connected neighbors may facilitate the higher quality concept embeddings. 
%coverage is not the only factor we should consider when selecting the knowledge graphs.

\begin{table}
    
    \caption{\label{tab:retrieved_concepts_statistics} Statistics for average question and answer tokens of three datasets.}
\end{table}



    
\section{randomless}


one insight: 
SWOW could be an adequent alternative to ConceptNet 

ELMO
Glove 
BERT 
how much knowledge 
what kinds of knowledge beyond text are in ConceptNet and SWOW? 
ConceptNet is a big, it doesn't translate to other language easily
SWOW is simpler architecture, SWOW is easier to sc


Some and interpreable 

Which of the two is best in commonsense question answering tasks? 

-------------

we show that X improves upon Y (because Z)

. In this paper, we introduce the ConSeqNet
framework, which enables the use of various kinds of external knowledge bases to retrieve knowledge relevant to
a given NLI instance, by retrieving information related to
the premise and hypothesis. 

We describe our novel architecture and demonstrate its use with a specific external knowledge source – ConceptNet – and evaluate its performance on
two other sources, WordNet and DBpedia. 
We compare the performance of three distinct approaches to augmenting the
knowledge used to train for and to predict entailment relationships between given pairs of premises and hypotheses:
graph-only, text-only, and text-and-graph. Using both qualitative and quantitative results, we demonstrate that introducing graph-based features boosts performance on the NLI
problem, but only when text features are present as well. Our
system has a competitive performance (accuracy) of 85.2\%
on the SciTail entailment dataset, which is derived from science domain question answering datasets.



Q2. Can Knowledge Graph embeddings trained on SWOW bring additional improvements on text encoder? 
Two aspects: 
\begin{enumerate}
    \item Why adding GconAttn on the top of BiLSTM drops the performance? 
    BiLSTM + OBQA 
    BiLSTM + GconAttn + OBQA

    Text: Glove + OBQA/CSQA 
    Glove+GconAttn + 

    
    \item How can I verify this with a simple model?
\end{enumerate}


key problem:
I need a baseline for CSQA. (ESIM, BiLSTM, or glove ) and then proove add kg on the baseline can improve the performance.
the official code provides the ESIM code, (SWAG also provide the glove and number batch code)

I will use the split of (Lin 2019) on ESIM, get the baseline results. 
\end{comment}

==> body/scribble.tex <==

what's the problem?

topic: Whether we can make use of free word associations for commonsense question answering?


The problem is that relational commonsense knowledge is difficult to collect,

free word associations is a easier way of collect commonsense knowledge,
knowledge collected in this way can be used for commonsense reasoning (use an example to show this.) 

Although 
Most knowledge in ConceptNet comes from the 

Commonsense knowledge in ConceptNet are usually collected in three ways, including hand-crafted by experts, automatically extracted from the Web, and games with a purpose. 

The problem is commonsense knowledge is difficult to collect, even though automatic mining techniques are used to mine commonsense knowledge from the web




1.  state the problem from 
current KG-aware models usually use knowledge graph embedding techniques to pre-train entities and relations in a knowledge graph and incorporate them into a question-answer model

using commonsense knowledge can enhance the reasoning ability 


current KG-aware model pipeline: 

KG -> KG Embeddings -> QA model 


So, let me summarise (and correct me if I'm wrong):
we consider 3 data sets
we consider a very simple embedding method (TransE) and a fairly simple, but competitive, KG/text integration method
SWOW and CN perform very similarly across datasets
Across data sets, both give some improvement over language models of varying strength

Based on what we have, here's how I see this going forward:
For a quick paper, all we could say is that SWOW seems to be a promising alternative to CN for KG-based common sense reasoning; which is not too bade, motivating further research
Even a quick paper should perhaps include experiments using SWOW+CN combined to probe for complementarity
if we wanted to strengthen the paper we could explore stronger KG embedding models and / or another language


step1: where should I start?
what options do I have? 

introduction 
related work?
experimental results analysis:


step2: Just do it! 

What is the  


What's your contribution?

==> figures/shortest_path_sw_183.tex <==
\tikzstyle{start}=[rectangle, draw,thick, text centered, rounded corners, minimum height=1em,draw, text width=8mm]
\tikzstyle{middle}=[rectangle, draw, dashed, text centered, rounded corners, minimum height=1em,draw, thick, text width=8mm]
\tikzstyle{end}=[rectangle, draw, thick, text centered, rounded corners, minimum height=1em,draw, thick,text width=8mm]

\tikzstyle{swow}=[rectangle, draw,thick,
    text centered, rounded corners, minimum height=0.8em,draw=cyan!50,fill=cyan!20]
\tikzstyle{cpnet}=[rectangle, draw,thick,
    text centered, rounded corners, minimum height=0.8em,draw=blue!50,fill=blue!20]
\tikzstyle{cpsw}=[rectangle, draw,thick,
    text centered, rounded corners, minimum height=0.8em,draw=green!50,fill=green!20]
    
\pgfplotsset{compat=newest}
\tikzstyle{annotation} = [rectangle, draw=none, fill=none, text centered, rounded corners]

\begin{figure}[!t]
    \begin{adjustbox}{width=0.3\columnwidth}
	\begin{tikzpicture}
% 	\draw[help lines, dashed] (-5,-4) grid (4,4);
% S grow -> veggy
% S grow -> plant
% S grow -> weed
% S water -> garden
% S continue -> pick
% S bee -> pollinate
% S bee -> fly -> arrive
% S cover -> band -> hole
% S begin -> blossom -> ripen
% S flower -> become -> appear
% S continue -> stick -> pick
% S n/a
% S start -> green -> grow -> veggie
    
    \node [start, text width=8mm, align=center] (grow) at (-0.5,0) {grow};
    \node [end, right of= grow, node distance=1cm, xshift=8mm, align=center] (vegetable) {vegetable};
    \path[->, thick, draw=blue!50, fill=blue!50,] (grow)  edge  node[sloped, anchor=auto, above, scale=0.8,font=\small] {}  (vegetable);
    
    \node [end, below of= vegetable, node distance=1cm,align=center] (plant) {plant};
    \path[->, thick, draw=blue!50, fill=blue!50,] (grow)  edge  node[sloped, anchor=auto, above, scale=0.8,font=\small] {}  (plant);
    
    \node [end, below of= plant, node distance=1cm,align=center] (weed) {weed};
    \path[->, thick, draw=blue!50, fill=blue!50,] (grow)  edge  node[sloped, anchor=auto, above, scale=0.8,font=\small] {}  (weed);
    
    \node [end, below of= grow, node distance=3cm,align=center] (water) {water};
    \node [end, below of= weed, node distance=1cm,align=center] (garden) {garden};
    \path[->, thick, draw=blue!50, fill=blue!50,] (water)  edge  node[sloped, anchor=auto, above, scale=0.8,font=\small] {}  (garden);
    
    \node [end, below of= grow, node distance=4cm,align=center] (bee) {bee};
    \node [end, below of= vegetable, node distance=3cm,align=center] (pollinate) {pollinate};
    \path[->, thick, draw=blue!50, fill=blue!50,] (bee)  edge  node[sloped, anchor=auto, above, scale=0.8,font=\small] {}  (pollinate);
    
	\end{tikzpicture}
% 	}
    \end{adjustbox}
% 	\end{subfigure}
	\caption{\label{fig:camping_cn_sw} Sub-graphs centered around ``\textbf{camping}'' from (a)~\cn and (b)~\swow. Nodes in green are common to both KGs. Nodes on the left/blue (right/cyan) are unique to \cn (\swow). 
% 	\lea{something like this? Shall we have about the same CN as SW associations? And: Sec 2 says that SW has more bigrams than CN. It's unfortunate if the figure suggests the opposite ;) Try to show some of the points you discuss in S2.}
	}
\end{figure}
% \end{comment}


==> tables/grounded_kg_overlap_cn_sw.tex <==

\begin{comment}
\begin{table}[!h]
    \centering
    % \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{p{2.7cm}ccc}
	\toprule
	  & KG & CSQA & OBQA \\
	\hline
% 	\multirow{3}{*}{Nodes} & CN & 24,636 & 18,764 \\
% 	 & SW & 16,536 & 14,179 \\
% 	 overlap & 15,241 & 12,661 \\\hline
	 \multirow{2}{2.7cm}{Node overlap (\%)} & {\tiny \cn} & 61.86 & 67.47 \\
	 & {\tiny \swow} & 92.16 & 89.29 \\\hline
% 	\multirow{2}{*}{\#Paths} & CN & 2,344,377 & 902,870 \\
% 	 & SW & 4,070,017 & 1,829,925 \\\hline
	\multirow{2}{2.7cm}{Link overlap (\%)} & {\tiny \cn} & 30.38 & 98.28 \\
	 & {\tiny \swow} & 26.83 & 99.14 \\
	\bottomrule
    \end{tabular}
    % \end{adjustbox}
    \caption{Comparisons of overlap nodes and links between \cn and \swow on CSQA and OBQA. }
    \label{tab:grounded_kg_cn_sw}
\end{table}
\end{comment}

\begin{table}[!ht]
    \centering
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{p{2cm}lll}
	\toprule
	 & KG & CSQA & OBQA \\
	\hline
	\multirow{3}{*}{\#Nodes} & CN & 24,636 & 18,764 \\
	 & SW & 16,536 & 14,179 \\
	 & Overlap & 15,241 & 12,661 \\\hline
	\multirow{2}{*}{\#Paths} & CN & 2,344,377 & 902,870 \\
	 & SW & 4,070,017 & 1,829,925 \\\hline
	\multirow{2}{2cm}{Overlap \\Connectivity} & CN(\%) & 30.38 & 98.28 \\
	 & SW(\%) & 26.83 & 99.14 \\
	\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Comparisons of grounded nodes and paths between \cn and \swow on CSQA and OBQA. Overlap connectivity indicates whether two common nodes are connected (1hop or 2hop). }
    \label{tab:grounded_kg_cn_sw}
\end{table}


\begin{comment}
\begin{table}[!ht]
    \centering
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{l|ccc|cc|cc}
	\toprule
	  & \multicolumn{3}{|c}{\#Nodes} & \multicolumn{2}{|c}{\#Paths} &  \multicolumn{2}{|c}{Overlap Connectivity} \\
	 Dataset & CN & SW & Overlap & CN & SW & CN(\%) & SW(\%) \\ \midrule
    CSQA & 24,636 & 16,536 & 15,241 & 2,344,377 & 4,070,017 & 30.38 & 26.83 \\
	OBQA & 18,764 & 14,179 & 12,661 & 902,870 & 1,829,925 & 98.28 & 99.14 \\
    
    % Dataset CN SW Overlap CN SW CN(\textbackslash \%) SW(\textbackslash \%)
% 	CSQA & 24,636 & 16,536 & 15,241 & 2,344,377 & 4,070,017 & 712,162 & 1,091,825 \\
% 	OBQA & 18,764 & 14,179 & 12,661 & 902,870 & 1,829,925 & 887,337 & 1,814,139 \\
% 	CSQA & 19,533 & 14,364 & 4,207 & 2,344,377 & 4,070,017 & 712,162 & 1,091,825 \\
% 	OBQA & 11,778 & 10,994 & 8,793 & 902,870 & 1,829,925 & 887,337 & 1,814,139 \\
	\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\CN (CN) and \SWow (SW) grounded nodes and paths on Commonsense QA and OpenbookQA. Overlap connectivity indicates whether two nodes from the overlap nodes are connected (1hop or 2hop). }
    \label{tab:local_kg_CN_SW}
\end{table}

\end{comment}







\begin{comment}
\begin{table}[!ht]
    \centering
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{lll|ll}
	\toprule
	& \multicolumn{2}{c|}{Node overlap} & \multicolumn{2}{c}{Path overlap}  \\
% 	\midrule
	Dataset & CN(\%) & SW(\%) & CN(\%) & SW(\%) \\\hline
	CSQA & 21.54 & 29.29 & 30.38 & 26.83 \\
	OBQA & 74.66 & 79.98 & 98.28 & 99.14 \\
	\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Overlap ratio of grounded nodes and paths on Commonsense QA and OpenbookQA. \ch{Not sure Table4 and Table5, which one is better?}
    \label{tab:local_kg_overlap_CN_SW}}
\end{table}
\end{comment}

==> tables/kg_coverage_edge_node.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% nx.MultiDiGraph()
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[th]
\begin{adjustbox}{width=0.48\textwidth}
% \small
\large
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{4}{l}{\textbf{Target KG$\rightarrow{}$}}\\
 \cmidrule{2-5}
\textbf{Source KG$\downarrow{}$}   & \multicolumn{2}{c}{Pairs} & \multicolumn{2}{c}{Nodes} \\
& \cn & \sw& \cn & \sw \\
\midrule                  
\cn     & -        & 4.7\%      & -  & 6.7\%  \\
\sw & 9.6\%   & -           & 57.8\%  & -   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\label{tab:kg_coverage_edge_node} \textbf{Edge and node coverage} - The proportion of (head, tail) pairs and nodes in a Source KG is found in a Target KG.} 
% \begin{equation}
%     p = N_{\cnisw}/N_{target KG}
% \end{equation}
\end{table}



%   direction  edge_precison  node_precision  source(node, edge)  target(node, edge) intersection(node, edge)
% 0    CN->SW          0.047           0.067  (1080759, 3009636)   (124626, 1593564)          (71975, 140249)
% 0    SW->CN          0.096           0.578   (124626, 1593564)  (1080759, 3009636)          (71975, 153481)


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% nx.Graph()
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[th]
% \begin{adjustbox}{width=0.48\textwidth}
% % \small
% \large
% \begin{tabular}{lcccc}
% \toprule
%  & \multicolumn{4}{l}{\textbf{Target KG$\rightarrow{}$}}\\
%  \cmidrule{2-5}
% \textbf{Source KG$\downarrow{}$}   & \multicolumn{2}{c}{Pairs} & \multicolumn{2}{c}{Nodes} \\
% & \cn & \sw& \cn & \sw \\
% \midrule                  
% \cn     & -        & 6.3\%      & -  & 6.7\%  \\
% \sw & 14.6\%   & -           & 57.8\%  & -   \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\label{tab:kg_coverage_edge_node} \textbf{Edge and node coverage} - The proportion of (head, tail) pairs and nodes in a Source KG is found in a Target KG.} 
% % \begin{equation}
% %     p = N_{\cnisw}/N_{target KG}
% % \end{equation}
% \end{table}


% direction  edge_precison  node_precision  source(node, edge)  target(node, edge) intersection(node, edge)
% 0    CN->SW          0.063           0.067  (1080759, 3009636)   (124626, 1593564)          (71975, 190212)
% 0    SW->CN          0.146           0.578   (124626, 1593564)  (1080759, 3009636)          (71975, 232442)



==> tables/learning_rate.tex <==
\begin{table*}
    \centering
    %\footnotesize
    %\begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{llll}
	\toprule
	 & CommonsenseQA & OpenbookQA & MCScript2.0 \\
	\midrule
	Albert-xxlarge-v2 & 1.00E-05 & 1.00E-05 &  1.00E-05\\
	RoBERTA-Large & 2.00E-06 & 1.00E-05 & -\\
	\midrule
		GconAttn & 3.00E-04 & 3.00E-04  & 1.00E-03\\
	RN & 1.00E-03 & 3.00E-04 & 1.00E-03 \\
	\bottomrule
    \end{tabular}
    %\end{adjustbox}
    \caption{Learning rate for various text encoders (top), and KG-augmented models (bottom).}
    \label{tab:text_encoders_learning_rate}
\end{table*}



==> tables/node_pair_pos_phrase_ratio_cn_sw.tex <==

\begin{table}
    \centering
    \begin{tabular}{lll}
	\toprule
	Node Pair Type & ConceptNet & SWOW \\
	\midrule
	word-word & 0.7040 & 0.9094 \\
	word-phrase & 0.2268 & 0.0859 \\
	phrase-phrase & 0.0657 & 0.0016 \\
	\bottomrule
    \end{tabular}
    \caption{\label{tab:node_pair_pos_phrase_ratio_cn_sw} The proportion of node pair type (POS and Phrase type) combinations.}


\end{table}



\begin{comment}
	
\begin{table}
    \centering
    \begin{tabular}{lll}
	\toprule
	PhraseTypes & ConceptNet & SWOW \\
	\midrule
	PosPos & 0.6235 & 0.8839 \\
	PosPhrase & 0.2604 & 0.1091 \\
	PhrasePhrase & 0.1129 & 0.0033 \\
	\bottomrule
    \end{tabular}
    \caption{\label{tab:node_pair_pos_phrase_ratio_cn_sw} The proportion of node pair type (POS and Phrase type) combinations.}

\end{table}
\end{comment}

==> tables/node_phrase_type.tex <==
\begin{table}[htbp]
    \centering    
    \begin{tabular}{ccc}
        \toprule
        Phrase Type & \texttt{ConceptNet} & \texttt{SWOW} \\
        \midrule
         NP & \textbf{0.7867} & 0.7216 \\
        VP & 0.0653 &  \textbf{0.0988} \\
        ADJP & 0.0453 & \textbf{0.0705} \\
        ADVP & \textbf{0.0138} & 0.0123 \\
        PP & 0.006 &  \textbf{0.0163} \\
        Others & 0.0829 & 0.0805 \\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:node_phrase_type} Node phrase types }
\end{table}
\smallskip


==> tables/qa_datasets_statistics.tex <==
\begin{table}[!ht]{
    \begin{adjustbox}{width=0.45\textwidth}
    \small
    \begin{tabular}[width=\textwidth]{lcccc}
        \toprule
         Datasets& Train & Dev & Test  \\
        \midrule
        CommonsenseQA & 8,500 & 1,221 & 1,241 \\
        OpenBookQA & 4,957 & 500 & 500 \\
        % SocialIQA & 33,410 & 1,954 & 2,224 & 3 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\label{tab:qa_datasets_statistics} Statistics of three commonsense question answering datasets.}
    %* uses the split from \citep{Lin2019KagNetKG}. %C denotes the number of choices.
    }
\end{table}
\smallskip

